Towards the Inferrence of Structural Similarity of Combinatorial Landscapes

One of the most common problem-solving heuristics is by analogy. For a given problem, a solver can be viewed as a strategic walk on its fitness landscape. Thus if a solver works for one problem instance, we expect it will also be effective for other instances whose fitness landscapes essentially share structural similarities with each other. However, due to the black-box nature of combinatorial optimization, it is far from trivial to infer such similarity in real-world scenarios. To bridge this gap, by using local optima network as a proxy of fitness landscapes, this paper proposed to leverage graph data mining techniques to conduct qualitative and quantitative analyses to explore the latent topological structural information embedded in those landscapes. By conducting large-scale empirical experiments on three classic combinatorial optimization problems, we gain concrete evidence to support the existence of structural similarity between landscapes of the same classes within neighboring dimensions. We also interrogated the relationship between landscapes of different problem classes.

==> backups/introductionv_5_18_1.tex <==
\section{Introduction}
\label{sec:introduction}


\IEEEPARstart{B}{lack-box} optimization problems (BBOPs), originated from black-box concepts in cybernetics, aims at finding a solution $\mathbf{x} \in \mathbb{R}^n$ that maximizes or minimizes an objective value $f(\mathbf{x})$ without any explicit knowledge of the objective function $f: \mathbb{R}^n \to \mathbb{R}$. Such problems are often encounterd in various scenarios in real-world engineering. For instance, in the field of hyperparameter optimization, the tunning of machine learning models is often formulated as a BBOP, where the objective is to minimize the prediction loss by properly assigning values to a set of hyperparameters~\cite{FeurerH19}. In software engineering, many modern software systems and programs are highly customizable, allowing users to tailor them to a specific application scenario. In this context, the task of finding an optimal configuration of the software to maximize certain performance aspects could also be considered as a BBOP~\cite{WeberAS21}. Since there does not exist any analytical form or authentic solution for a BBOP, it is hard to interpret and investigate except for an observation of input-output response through experimentation.

In evolutionary and meta-heuristic optimization, the fitness landscape~\cite{Wright1932} metaphor has been extensively used to understand the relationships between algorithm performance and underlying properties of BBOPs. For a given problem, a solver's search behavior could be considered as a strategic walk along the corresponding fitness landscape. Therefore, the performance of a BBOP solver would thus highly depend on the structures of the underlying landscape, which makes the \textit{structural characteristics} of BBOP landscapes an active area of research. In particular, there has been evidence suggesting that certain patterns or structures are associated with the fitness landscape of a BBOP, rather than a full randomness. For example, \dots. At a higher level, Tayarani-N and Pr{\"{u}}gel{-}Bennett compared the landscape characteristics of four classic BBOPs. Though ambiguous, their results indicated that though superficially different, the fitness landscapes of those problems share certain level of similarities~\cite{TayaraniP14}.

Analogy is one of the most common problem-solving approaches in practice. In the context of BBOP, its basic assumption is that if a BBOP solver is effective for one problem, we could then expect its effectiveness for solving other problems whose fitness landscapes essentially share \textit{structural similarity} with each other. In other words, the strategic walk on the fitness landscapes induced by the solver may be extended to landscapes of similar problems that are anticipated to share certain patterns or sub-structures but vary in different sizes or volumes. Thereby, when encountering a novel BBOP instance $P_0$, we could follow an analogical reasoning process to study it, which typically consists of three tasks~\cite{Gentner83, ThagardHNG90}:


\begin{itemize}
    \item \textit{Retrieval}: select a set of candidate analogous instances $\mathcal{P} = \{P_1, \dots, P_k\}$.
    \item \textit{Judgement}: determine the similarity $\mathrm{Sim}(P_i,P_j)$ between each distinct pair of instances  $(P_i, P_j)\in\mathcal{P}^2$ based on a similarity function $\mathrm{Sim}: \mathcal{P} \times \mathcal{P} \rightarrow [0, 1]$ (and thus obtain a similarity matrix $\mathbf{S}$ as shown in \pref{fig:matrix}).
    \item \textit{Inference}: apply knowledge from the most analogous instance $\hat{P_0}$ to handle $P_0$, where $\mathrm{Sim}(\hat{P},P) \geq \max_{P' \in \mathcal{P}} \mathrm{Sim}(P',P_0)$ for $\forall P' \in \mathcal{P}$. Here, the specific knowledge applied would depend on tasks at hand.
\end{itemize}

\begin{figure}[t!]
    \centering
    \includegraphics[width=.45\linewidth]{figs/matrix.pdf}
    \caption{An example of similarity matrix $\mathbf{S}$ for a set of BBOP instances $\mathcal{P} = \{P_0, \dots, P_3\}$. A \enquote{$-$} in the diagonal entry indicates that is is meaningless to measure the similarity of an instance with itself. The upper trangular part of the matrix is symmetric to the lower one and is thus omitted for brevity.}
    \label{fig:matrix}
\end{figure}

At the core of the similarity function $\mathrm{Sim}$ is the structural similarity between the fitness landscapes of two BBOP instances. Since it would not only enable us to transfer our knowledge on a well-studied problem to solve previously unseen instances, but also deepen our understanding of the relationships between different problem instances, this brings a fundamental new pespective for studying BBOPs. 

However, in practice it is far from trivial to directly compare fitness landscapes when encountering BBOPs due to their abtract and extremely high-dimensional nature. In addition, the study in cogonitive science indicates that simply basing the similarity determination on the size of overlap between general object features are not appropriate since not all features are equally relevant to the interpretaion. Instead, only certain kinds of matches count for or against analogies, and higher-order relationships should be discovered~\cite{Gentner83}. For example, battery and reservoir are totally different things in many aspects (e.g., color, size shape and substance). However, at a higher level, their similary functions of storing and releasing energy makes it reasonble to consider them as analogous.

In the last three decades and beyond, considerable efforts have been devoted to developing methods for characterizing structural features of fitness landscape under both the term FLA and exploratory landscape analysis (ELA)~\cite{MersmannBTPWR11}. They have also been succesfully applied to guide the design and improvment of BBOP solvers, constitute feature vectors for automated algorithm selection and algorithm performance prediction, as well as gain insights into BBOPs themselves. 

In the more recent decade, among various newly developed methods for characterizing fitness landscapes, local optima networks (LONs) have become one of the most popular ones in the meta-heuristic community~\cite{Malan21}. LONs are rooted in the study of energy landscapes in chemical physics~\cite{Stillinger95} and its basic idea is to model the fitness landscape as a graph. In particular, the vertices of a LON are local optima and the edges indicate certain search dynamics of a meta-heuristic algorithm. As LON is able to capture various characteristics of the underlying landscape (e.g., the number of local optima, their distribution and connectivity pattern), it is a powerful tool for FLA~\cite{OchoaM19}.

More importantly, the graph nature of LON also makes it highly suitable for this pariticular study. 
% point 1
For example, the use of LONs allow us to take advantages of various metrics developed for complex networks~\cite{BoccalettiLMCH06} to analyze structural properties of the underlying landscapes. 
% point 2
In addition, with graph layout and dimensionality reduction methods, LONs are easy to visualize, enabling us to obtain an intuitive understanding of the typological structures of fitness landscapes~\cite{Graph_Visual_Survey1}.
% point 3
Morever, graph representation learning techniques, which have been widely used in the field of network science~\cite{ZhangYZZ20}, could be applied to obtain low-dimensional representations that are able to capture high-level structures of fitness landscapes. These could then be used to constitute a richer set of features for characterizing fitness landscapes.

Build on our recent work which conducted a case study on inferring the structural similarity of fitness landscapes across different dimensions of number partitioning problems (NPPs), in this study, we seek to gain further insights on a wider scope of landscapes with more comprehensive analysis. Specifically, we consider four types of classic BBOPs, inlcuding NPP, maximum satisfiability (Max-Sat), the traveling salesman problem (TSP), and the knapsack problem (KP). We seek to study the structural similarity of different problem instances at different levels, which lead us to our first three research questions (RQs). To start with, we also first consider problem instances of different dimensions. 

\begin{itemize}
    \item \textbf{\underline{RQ1}}: \textit{For each class of problems, can we investigate any potential structural similarity in fitness landscapes across instances of \underline{different dimensions?}}
    \item \textbf{\underline{RQ2}}: \textit{For each class of problems, can we investigate any potential structural similarity in fitness landscapes across instances of \underline{different sub-classes?}}
    \item \textbf{\underline{RQ3}}: \textit{Can we investigate any potential structural similarity in fitness landscapes across instances that belong to \underline{different classes} of problems?}
\end{itemize}

% \begin{tcolorbox}[sharpish corners, top=2pt, bottom=2pt, left=4pt, right=4pt, boxrule=0.0pt, colback=black!5!white, leftrule=0.75mm,]
%     \textbf{\underline{RQ1}:} \textit{For each class of problems, can we investigate any potential structural similarity in fitness landscapes across instances of different dimensions?}
% \end{tcolorbox}

% \begin{tcolorbox}[sharpish corners, top=2pt, bottom=2pt, left=4pt, right=4pt, boxrule=0.0pt, colback=black!5!white, leftrule=0.75mm,]
%     \textbf{\underline{RQ2}:} \textit{For each class of problems, can we investigate any potential structural similarity in fitness landscapes across instances of different sub-classes?}
% \end{tcolorbox}

% \begin{tcolorbox}[sharpish corners, top=2pt, bottom=2pt, left=4pt, right=4pt, boxrule=0.0pt, colback=black!5!white, leftrule=0.75mm,]
%     \textbf{\underline{RQ3}:} \textit{Can we investigate any potential structural similarity in fitness landscapes across instances of different classes of problems?}
% \end{tcolorbox}

The empirical results with regard to the first three RQs is highly inspiring, as we are able to disclose the similarities and differences between a wide range of instances by both qualitative and quantitative analysis. We then evalute the efficacy of our measured similarity by running heuristic algorithms on each problem instance. The rationale behind this particular analysis is based on the hypothesis that the level of similarity between two landscapes should be correlated with the performance difference of meta-heuristics on the corresponding problems, which leads to our final RQ: 

\begin{itemize}
    \item \textbf{\underline{RQ4}}: \textit{How effective is the measured similarity in explaining the performance difference of meta-heuristics between different problem instances?}
\end{itemize}

The experimental results show that the $Sim$ value could has a good correlation with performance differences of testing algorithms.

Details of our empirical experiments and responses to these RQs will be elaborated in later sections step by step. Drawing on these answers, this study, for the first time, provides new insights help to further advance this field of research. In a nutshell, the main contributions of this paper could be summarized as follows:

\begin{itemize}
    \item To the best of our knowledge, this work represents the first attempt to infer structure similarity between fitness landscapes of different COPs.
    \item We proposed a new fitness landscape visualization technique based on LON by leveraging node embedding and dimensionality reduction method.
    \item We developed a quantitative measure of structural similarity between different combinatorial landscapes using graph embedding technique and correlation metrics.
    \item We developed a \texttt{Python} package for performing graph-based landscape analysis. 

\end{itemize}

In the rest of this paper, \pref{sec:preliminaries} provides some preliminary knowledge related to this work. \pref{sec:method} delineates our empirical methodologies for problem instance generation and LON construction. Extensive empirical results are presented and analyzed in~\pref{sec:results}. In the end, \pref{sec:conclusions} concludes this paper and threads some light on future directions.

% The "No-Free-Lunch" Theorem
% Despite many successful BBOP solvers have been developed in different disciplines, the famous \enquote{No-Free-Lunch} theorem~\cite{DolpertM97} points out that there is no single algorithm that could always yield superior performance than others for all optimization problems. Therefore, in-depth understanding of the characteristics of the underlying BBOP is required to facilitate the design, selection as well as configuration of appropriate solvers for a given task.

% Under this paradigm, the task of finding an effective solver for a given problem instance could be transformed into the problem of finding a similar instance for which an effective solver is already known. At the core of this theory is a proper definition of the \textit{similarity} between problem instances, which is often based on representative features that are able to capture certain problem characteristics designed by domain experts.
% At the core of the analogical reasoning process is the judgement of \textit{similarity} between problems, which is often based on representative features that are able to capture certain problem characteristics designed by domain experts.

% While most of the existing works are dedicated to the study of a single type of BBOP, there has been evidence that the fitness landscapes of different BBOPs, although superficially different, may share certain patterns or sub-structures, rather than a full randomness~\cite{TayaraniP14}. 
% it is often the case that we are also interested in the relationship between different BBOP instances, i.e., is there any sharing of certain patterns or sub-structures among the fitness landscapes of different BBOPs?
% it is often the case that we are interested in the relationship between different problem instances. In fact, it has long been desired to answer the question of \enquote{what makes a BBOP hard?}. There have been attempts to classify BBOP instances into \enquote{hard} and \enquote{easy} ones~\cite{BrownNS09}. It has also been noted that although different at the surface, the fitness landscapes of different BBOPs may share certain patterns or structures, rather than a total disimilarity~\cite{TayaraniP14}. 

% Its fundamental premise is that if two problems share certain similarities with each other, then the problem-solving strategy effective for one problem would possibly also be useful for the other one. 
% In the context of BBOP, it is often the case in real world scenarios that we may encounter a problem instance which could be essentially similar to well-known problem. 

% \begin{figure}[t]
%     \centering
%     $\mathbf{S}=
%     \begin{blockarray}{*{4}{c} l}
%       \begin{block}{*{4}{>{$\footnotesize}c<{$}} l}
%         $P_0$ & $P_1$ & $P_2$ & $P_3$ & \\
%       \end{block}
%       \begin{block}{[*{4}{c}]>{$\footnotesize}l<{$}}
%         - & $\times$ & $\times$ & $\times$  \bigstrut[t]& $P_0$ \\
%         0.9 & - & $\times$ & $\times$  & $P_1$ \\
%         0.7 & 0.8 & - & $\times$  & $P_2$ \\
%         0.4 & 0.5 & 0.6 & -  & $P_3$ \\
%       \end{block}
%     \end{blockarray}$
%     \caption{An example of similarity matrix $\mathbf{S}$ for a set of four BBOP instances.}
%     \label{fig:similarity_matrix}
% \end{figure}


==> backups/introductionv_5_18_2.tex <==
\section{Introduction}
\label{sec:introduction}


\IEEEPARstart{B}{lack-box} optimization problems (BBOPs), originated from black-box concepts in cybernetics, aims at finding a solution $\mathbf{x} \in \mathbb{R}^n$ that maximizes or minimizes an objective value $f(\mathbf{x})$ without any explicit knowledge of the objective function $f: \mathbb{R}^n \to \mathbb{R}$. Such problems are often encounterd in various scenarios in real-world engineering such as economics, machine learning and software engineering, etc. 
Despite many sucessful BBOP solvers hav been developed in different disciplines, the famous \enquote{No-Free-Lunch} theorem~\cite{DolpertM97} points out that there is no single algorithm that could always yield superior perfromance than others for all optimization problems. Therefore, in-depth understanding of the characteristics of the underlying BBOP is essential to facilitate the design, selection and configuration of appropriate solvers for a given task. However, since there does not exist any analytical form or authentic solution for a BBOP, it is hard to interpret and investigate except for an observation of input-output response through experimentation.

In practice, analogy is one of the most common problem-solving approaches, and it is particularly helpful for the understanding of abtract, complex systems~\cite{RichlandS15}. In the context of BBOP, its basic assumption is that if a BBOP solver is effective for one problem, we could then expect its effectiveness for solving other problems which essentially share \textit{similarity} with each other. Thereby, when encountering a novel BBOP instance $P_0$, we could follow an analogical reasoning process to study it, which typically consists of three tasks~\cite{Gentner83, ThagardHNG90}:

\begin{itemize}
    \item \textit{Retrieval}: select a set of candidate analogous instances $\mathcal{P} = \{P_1, \dots, P_k\}$.
    \item \textit{Judgement}: determine the similarity $\mathrm{Sim}(P_i,P_j)$ between each distinct pair of instances  $(P_i, P_j)\in\mathcal{P}^2$ based on a similarity function $\mathrm{Sim}: \mathcal{P} \times \mathcal{P} \rightarrow [0, 1]$ (and thus obtain a similarity matrix $\mathbf{S}$ as shown in \pref{fig:matrix}).
    \item \textit{Inference}: apply knowledge from the most analogous instance $\hat{P_0}$ to handle $P_0$, where $\mathrm{Sim}(\hat{P},P) \geq \max_{P' \in \mathcal{P}} \mathrm{Sim}(P',P_0)$ for $\forall P' \in \mathcal{P}$. Here, the specific knowledge applied would depend on tasks at hand.
\end{itemize}

\begin{figure}[t!]
    \centering
    \includegraphics[width=.45\linewidth]{figs/matrix.pdf}
    \caption{An example of similarity matrix $\mathbf{S}$ for a set of BBOP instances $\mathcal{P} = \{P_0, \dots, P_3\}$. A \enquote{$-$} in the diagonal entry indicates that is is meaningless to measure the similarity of an instance with itself. The upper trangular part of the matrix is symmetric to the lower one and is thus omitted for brevity.}
    \label{fig:matrix}
\end{figure}

The inferrence of such similarity would not only enable us to transfer our knowledge on a well-studied problem to solve previously unseen instances, but also deepen our understanding of the relationships between different problem instances, and thus brings a fundamental new pespective for studying BBOPs. However, in practice it is far from trivial to directly infer such similarity when encountering BBOPs due to their black-box nature. In addition, study in cogonitive science states that not all features are equally relevant to the interpretaion. Intead, only certain kinds of matches count for or against analogies, and higher-order relationships should be discovered~\cite{Gentner83}. It is then important to \dots.
% For example, battery and reservoir are totally different things in many aspects (e.g., color, size shape and substance). However, at a higher level, their similary functions of storing and releasing energy makes it reasonble to consider them as analogous.

In evolutionary and meta-heuristic optimization, the fitness landscape~\cite{Wright1932} metaphor and its analysis (known as fitness landscapes analysis, FLA) have been extensively used to understand the underlying properties of BBOPs. In particular, the \textit{structures} of BBOP landscapes are found to be able to reflect important properties of problem instances and indicative to the overall performance of heuristic solvers. This is reasonable since for a given problem, a solver's search behavior could be considered as a strategic walk along the corresponding fitness landscape. Therefore, the performance of a BBOP solver would highly depend on the \textit{structural characteristics} of the underlying landscape.

In the last three decades and beyond, considerable efforts have been devoted to developing methods for characterizing such features of fitness landscape under both the term FLA and exploratory landscape analysis (ELA)~\cite{MersmannBTPWR11}, and they have enabled numerous new insights into the relationships between different BBOP instances. In particular, there has been evidence suggesting that certain patterns or structures are associated with the fitness landscape of a BBOP, rather than a full randomness. For example, \dots. At a higher level, Tayarani-N and Pr{\"{u}}gel{-}Bennett compared the landscape characteristics of four classic BBOPs. Though ambiguous, their results indicated that though superficially different, the fitness landscapes of those problems share certain level of similarities~\cite{TayaraniP14}.

In the more recent decade, among various newly developed methods for characterizing fitness landscapes, local optima networks (LONs) have become one of the most popular ones in the meta-heuristic community~\cite{Malan21}. LONs are rooted in the study of energy landscapes in chemical physics~\cite{Stillinger95} and its basic idea is to model the fitness landscape as a graph. In particular, the vertices of a LON are local optima and the edges indicate certain search dynamics of a meta-heuristic algorithm. The graph nature of LON makes it highly suitable for studying the structural characteristics of fitness landscapes, as it allows us to take advantages of various tools developed in the complex network community to effectively analyze fitness landscapes. 
% point 1
For example, metrics developed for complex networks~\cite{BoccalettiLMCH06} could be applied to analyze structural properties of the underlying landscapes. 
% point 2
In addition, graph layout and node embedding techniques would enable us to obtain intuitive visualizations of the typological structures of fitness landscapes~\cite{Graph_Visual_Survey1}.
% point 3
Morever, graph representation learning techniques~\cite{ZhangYZZ20} are able to extract low-dimensional representations that could capture high-level structures of fitness landscapes, which have shown efficacy in the determination of structural similarity between different fitness landscapes. 

Build on our recent work which conducted a case study on inferring the structural similarity of fitness landscapes across different dimensions of number partitioning problems (NPPs), in this study, we seek to gain further insights on a wider scope of landscapes with more comprehensive analysis. Specifically, we consider four types of classic BBOPs, inlcuding NPP, maximum satisfiability (Max-Sat), the traveling salesman problem (TSP), and the knapsack problem (KP). We seek to study the structural similarity of different problem instances at different levels, which lead us to our first three research questions (RQs). To start with, we also first consider problem instances of different dimensions. 

\begin{itemize}
    \item \textbf{\underline{RQ1}}: \textit{For each class of problems, can we investigate any potential structural similarity in fitness landscapes across instances of \underline{different dimensions?}}
    \item \textbf{\underline{RQ2}}: \textit{For each class of problems, can we investigate any potential structural similarity in fitness landscapes across instances of \underline{different sub-classes?}}
    \item \textbf{\underline{RQ3}}: \textit{Can we investigate any potential structural similarity in fitness landscapes across instances that belong to \underline{different classes} of problems?}
\end{itemize}

% \begin{tcolorbox}[sharpish corners, top=2pt, bottom=2pt, left=4pt, right=4pt, boxrule=0.0pt, colback=black!20!white, leftrule=0.75mm,]
%     \textbf{\underline{RQ1}:} \textit{For each class of problems, can we investigate any potential structural similarity in fitness landscapes across instances of different dimensions?}
% \end{tcolorbox}

% \begin{tcolorbox}[sharpish corners, top=2pt, bottom=2pt, left=4pt, right=4pt, boxrule=0.0pt, colback=black!20!white, leftrule=0.75mm,]
%     \textbf{\underline{RQ2}:} \textit{For each class of problems, can we investigate any potential structural similarity in fitness landscapes across instances of different sub-classes?}
% \end{tcolorbox}

% \begin{tcolorbox}[sharpish corners, top=2pt, bottom=2pt, left=4pt, right=4pt, boxrule=0.0pt, colback=black!20!white, leftrule=0.75mm,]
%     \textbf{\underline{RQ3}:} \textit{Can we investigate any potential structural similarity in fitness landscapes across instances of different classes of problems?}
% \end{tcolorbox}

The empirical results with regard to the first three RQs is highly inspiring, as we are able to disclose the similarities and differences between a wide range of instances by both qualitative and quantitative analysis. We then evalute the efficacy of our measured similarity by running heuristic algorithms on each problem instance. The rationale behind this particular analysis is based on the hypothesis that the level of similarity between two landscapes should be correlated with the performance difference of meta-heuristics on the corresponding problems, which leads to our final RQ: 

\begin{itemize}
    \item \textbf{\underline{RQ4}}: \textit{How effective is the measured similarity in explaining the performance difference of meta-heuristics between different problem instances?}
\end{itemize}

% \begin{tcolorbox}[sharpish corners, top=2pt, bottom=2pt, left=4pt, right=4pt, boxrule=0.0pt, colback=black!20!white, leftrule=0.75mm,]
%     \textbf{\underline{RQ4}:} \textit{How effective is the measured similarity in explaining the performance difference of meta-heuristics between different problem instances?}
% \end{tcolorbox}

The experimental results show that the $Sim$ value could has a good correlation with performance differences of testing algorithms.

Details of our empirical experiments and responses to these RQs will be elaborated in later sections step by step. Drawing on these answers, this study, for the first time, provides new insights help to further advance this field of research. In a nutshell, the main contributions of this paper could be summarized as follows:

\begin{itemize}
	\item To the best of our knowledge, this work represents the first attempt to infer structure similarity between fitness landscapes of different COPs.
	\item We proposed a new fitness landscape visualization technique based on LON by leveraging node embedding and dimensionality reduction method.
    \item We developed a quantitative measure of structural similarity between different combinatorial landscapes using graph embedding technique and correlation metrics.
    \item We developed a \texttt{Python} package for performing graph-based landscape analysis. 
\end{itemize}

In the rest of this paper, \pref{sec:preliminaries} provides some preliminary knowledge related to this work. \pref{sec:method} delineates our empirical methodologies for problem instance generation and LON construction. Extensive empirical results are presented and analyzed in~\pref{sec:results}. In the end, \pref{sec:conclusions} concludes this paper and threads some light on future directions.

% The "No-Free-Lunch" Theorem
% Despite many successful BBOP solvers have been developed in different disciplines, the famous \enquote{No-Free-Lunch} theorem~\cite{DolpertM97} points out that there is no single algorithm that could always yield superior performance than others for all optimization problems. Therefore, in-depth understanding of the characteristics of the underlying BBOP is required to facilitate the design, selection as well as configuration of appropriate solvers for a given task.

% Under this paradigm, the task of finding an effective solver for a given problem instance could be transformed into the problem of finding a similar instance for which an effective solver is already known. At the core of this theory is a proper definition of the \textit{similarity} between problem instances, which is often based on representative features that are able to capture certain problem characteristics designed by domain experts.
% At the core of the analogical reasoning process is the judgement of \textit{similarity} between problems, which is often based on representative features that are able to capture certain problem characteristics designed by domain experts.

% While most of the existing works are dedicated to the study of a single type of BBOP, there has been evidence that the fitness landscapes of different BBOPs, although superficially different, may share certain patterns or sub-structures, rather than a full randomness~\cite{TayaraniP14}. 
% it is often the case that we are also interested in the relationship between different BBOP instances, i.e., is there any sharing of certain patterns or sub-structures among the fitness landscapes of different BBOPs?
% it is often the case that we are interested in the relationship between different problem instances. In fact, it has long been desired to answer the question of \enquote{what makes a BBOP hard?}. There have been attempts to classify BBOP instances into \enquote{hard} and \enquote{easy} ones~\cite{BrownNS09}. It has also been noted that although different at the surface, the fitness landscapes of different BBOPs may share certain patterns or structures, rather than a total disimilarity~\cite{TayaraniP14}. 

% Its fundamental premise is that if two problems share certain similarities with each other, then the problem-solving strategy effective for one problem would possibly also be useful for the other one. 
% In the context of BBOP, it is often the case in real world scenarios that we may encounter a problem instance which could be essentially similar to well-known problem. 

% \begin{figure}[t]
%     \centering
%     $\mathbf{S}=
%     \begin{blockarray}{*{4}{c} l}
%       \begin{block}{*{4}{>{$\footnotesize}c<{$}} l}
%         $P_0$ & $P_1$ & $P_2$ & $P_3$ & \\
%       \end{block}
%       \begin{block}{[*{4}{c}]>{$\footnotesize}l<{$}}
%         - & $\times$ & $\times$ & $\times$  \bigstrut[t]& $P_0$ \\
%         0.9 & - & $\times$ & $\times$  & $P_1$ \\
%         0.7 & 0.8 & - & $\times$  & $P_2$ \\
%         0.4 & 0.5 & 0.6 & -  & $P_3$ \\
%       \end{block}
%     \end{blockarray}$
%     \caption{An example of similarity matrix $\mathbf{S}$ for a set of four BBOP instances.}
%     \label{fig:similarity_matrix}
% \end{figure}

==> backups/introductionv_5_18_3.tex <==

\section{Introduction}
\label{sec:introduction}


\IEEEPARstart{B}{lack-box} optimization problems (BBOPs), originated from black-box concepts in cybernetics, aims at finding a solution $\mathbf{x} \in \mathbb{R}^n$ that maximizes or minimizes an objective value $f(\mathbf{x})$ without any explicit knowledge of the objective function $f: \mathbb{R}^n \to \mathbb{R}$. Such problems are often encounterd in various scenarios in real-world engineering such as economics, machine learning and software engineering, etc. 
Despite many sucessful BBOP solvers have been developed in different disciplines, the famous \enquote{No-Free-Lunch} theorem~\cite{DolpertM97} points out that there is no single algorithm that could always yield superior perfromance than others for all optimization problems. Therefore, in-depth understanding of the characteristics of the underlying BBOP is essential to facilitate the design, selection and configuration of appropriate solvers for a given task. However, since there does not exist any analytical form or authentic solution for a BBOP, it is hard to interpret and investigate except for an observation of input-output response through experimentation.

In practice, analogy is one of the most common problem-solving approaches, and it is particularly helpful for the understanding of abtract, complex systems~\cite{RichlandS15}. In the context of BBOP, its basic assumption is that if a BBOP solver is effective for one problem, we could then expect its effectiveness for solving other problems which essentially share \textit{similarity} with each other. Thereby, when encountering a novel BBOP instance $P_0$, we could follow an analogical reasoning process to study it, which typically consists of three tasks~\cite{Gentner83, ThagardHNG90}:

\begin{itemize}
    \item \textit{Retrieval}: select a set of candidate analogous instances $\mathcal{P} = \{P_1, \dots, P_k\}$.
    \item \textit{Judgement}: determine the similarity $\mathrm{Sim}(P_i,P_j)$ between each distinct pair of instances  $(P_i, P_j)\in\mathcal{P}^2$ based on a similarity function $\mathrm{Sim}: \mathcal{P} \times \mathcal{P} \rightarrow [0, 1]$ (and thus obtain a similarity matrix $\mathbf{S}$ as shown in \pref{fig:matrix}).
    \item \textit{Inference}: apply knowledge from the most analogous instance $\hat{P_0}$ to handle $P_0$, where $\mathrm{Sim}(\hat{P},P) \geq \max_{P' \in \mathcal{P}} \mathrm{Sim}(P',P_0)$ for $\forall P' \in \mathcal{P}$. Here, the specific knowledge applied would depend on tasks at hand.
\end{itemize}

\begin{figure}[t!]
    \centering
    \includegraphics[width=.45\linewidth]{figs/matrix.pdf}
    \caption{An example of similarity matrix $\mathbf{S}$ for a set of BBOP instances $\mathcal{P} = \{P_0, \dots, P_3\}$. A \enquote{$-$} in the diagonal entry indicates that is is meaningless to measure the similarity of an instance with itself. The upper trangular part of the matrix is symmetric to the lower one and is thus omitted for brevity.}
    \label{fig:matrix}
\end{figure}

The inferrence of such similarity would not only enable us to transfer our knowledge on a well-studied problem to solve previously unseen instances, but also deepen our understanding of the relationships between different problem instances, and thus brings a fundamental new pespective for studying BBOPs. However, in practice it is far from trivial to directly infer such similarity when encountering BBOPs due to their black-box nature. 

In evolutionary and meta-heuristic optimization, the fitness landscape~\cite{Wright1932} metaphor and its analysis (known as fitness landscapes analysis, FLA) have been extensively used to understand the underlying properties of BBOPs. In particular, the \textit{structural characteristics} of BBOP landscapes are found to be able to reflect important properties of problem instances and indicative to the overall performance of heuristic solvers. This makes FLA a promising proxy for the inference of similarity between different BBOP instances. In other words, the strategic walk on the fitness landscapes of a solver might be extended to fitness landscapes 

In fact, there have been abundant evidence suggesting that certain patterns are associated with the landscape structure of a BBOP, and such patterns may share among different problem instances, or, even across different classess of problems~\cite{TayaraniP14}. However, despite many efforts, there has been no dedicated work to intuitively illustrate or quantitatively determine the \textit{structural similarity} between the fitness landscapes of different BBOP instances due to the lack of suitable analytical methods.

In the last three decades and beyond, considerable efforts have been devoted to developing statistical measures for characterizing fitness landscape, e.g., ruggendess, neutrality, epistasis variance and information content, etc. They have been successfully applied to guide the design and improvement of BBOP solvers, constitute feature vectors for automated algorithm selection and performance prediction, as well as gain insights into BBOPs themselves. However, in cogonitive science it is often the case that high-order relationships play a much more important role in determing the similarity between two instances. For example, whilst battery and reservoir are totally different things in many aspects (e.g., color, size shape and substance), at a higher level, their similary functions of storing and releasing energy makes it reasonble to consider them as analogous. It is thereby not sufficient to base our structural similarity inferrence only on hand-crafted features.

In the more recent decade, local optima networks (LONs) was proposed to model local optima in a fitness landscape and their transitions as a graph obejct. Specifically, the vertices of a LON are local optima and the edges indicate certain search dynamics of a meta-heuristic algorithm. Since LONs are able to capture various characteristics of the underlying landscape (e.g., the number of local optima, their distribution and connectivity pattern), they are powerful tools for fitness landscape analysis. In particular, the graph nature of LON makes it highly suitable for studying the structural characteristics of fitness landscapes. Notably, graph layout and node embedding techniques would enable us to obtain intuitive visualizations of the typological structures of fitness landscapes and make comparison between them~\cite{HuangL23}. In addition, Morever, graph representation learning techniques~\cite{ZhangYZZ20} are able to extract low-dimensional representations that could capture high-level structures of fitness landscapes, which have shown efficacy in the determination of structural similarity between different fitness landscapess~\cite{HuangL23}. 

% % point 1
% For example, metrics developed for complex networks~\cite{BoccalettiLMCH06} could be applied to analyze structural properties of the underlying landscapes. 
% % point 2
% In addition, graph layout and node embedding techniques would enable us to obtain intuitive visualizations of the typological structures of fitness landscapes~\cite{Graph_Visual_Survey1}.
% % point 3
% Morever, graph representation learning techniques~\cite{ZhangYZZ20} are able to extract low-dimensional representations that could capture high-level structures of fitness landscapes, which have shown efficacy in the determination of structural similarity between different fitness landscapes. 

Build on our recent work which conducted a case study on inferring the structural similarity of fitness landscapes across different dimensions of number partitioning problems (NPPs), in this study, we seek to gain further insights on a wider scope of landscapes with more comprehensive analysis. Specifically, we consider four types of classic BBOPs, inlcuding NPP, maximum satisfiability (Max-Sat), the traveling salesman problem (TSP), and the knapsack problem (KP). We seek to study the structural similarity of different problem instances at different levels, which lead us to our first three research questions (RQs). To start with, we also first consider problem instances of different dimensions. 

\begin{itemize}
    \item \textbf{\underline{RQ1}}: \textit{For each class of problems, can we investigate any potential structural similarity in fitness landscapes across instances of \underline{different dimensions?}}
    \item \textbf{\underline{RQ2}}: \textit{For each class of problems, can we investigate any potential structural similarity in fitness landscapes across instances of \underline{different sub-classes?}}
    \item \textbf{\underline{RQ3}}: \textit{Can we investigate any potential structural similarity in fitness landscapes across instances that belong to \underline{different classes} of problems?}
\end{itemize}

% \begin{tcolorbox}[sharpish corners, top=2pt, bottom=2pt, left=4pt, right=4pt, boxrule=0.0pt, colback=black!20!white, leftrule=0.75mm,]
%     \textbf{\underline{RQ1}:} \textit{For each class of problems, can we investigate any potential structural similarity in fitness landscapes across instances of different dimensions?}
% \end{tcolorbox}

% \begin{tcolorbox}[sharpish corners, top=2pt, bottom=2pt, left=4pt, right=4pt, boxrule=0.0pt, colback=black!20!white, leftrule=0.75mm,]
%     \textbf{\underline{RQ2}:} \textit{For each class of problems, can we investigate any potential structural similarity in fitness landscapes across instances of different sub-classes?}
% \end{tcolorbox}

% \begin{tcolorbox}[sharpish corners, top=2pt, bottom=2pt, left=4pt, right=4pt, boxrule=0.0pt, colback=black!20!white, leftrule=0.75mm,]
%     \textbf{\underline{RQ3}:} \textit{Can we investigate any potential structural similarity in fitness landscapes across instances of different classes of problems?}
% \end{tcolorbox}

The empirical results with regard to the first three RQs is highly inspiring, as we are able to disclose the similarities and differences between a wide range of instances by both qualitative and quantitative analysis. We then evalute the efficacy of our measured similarity by running heuristic algorithms on each problem instance. The rationale behind this particular analysis is based on the hypothesis that the level of similarity between two landscapes should be correlated with the performance difference of meta-heuristics on the corresponding problems, which leads to our final RQ: 

\begin{itemize}
    \item \textbf{\underline{RQ4}}: \textit{How effective is the measured similarity in explaining the performance difference of meta-heuristics between different problem instances?}
\end{itemize}

% \begin{tcolorbox}[sharpish corners, top=2pt, bottom=2pt, left=4pt, right=4pt, boxrule=0.0pt, colback=black!20!white, leftrule=0.75mm,]
%     \textbf{\underline{RQ4}:} \textit{How effective is the measured similarity in explaining the performance difference of meta-heuristics between different problem instances?}
% \end{tcolorbox}

The experimental results show that the $Sim$ value could has a good correlation with performance differences of testing algorithms.

Details of our empirical experiments and responses to these RQs will be elaborated in later sections step by step. Drawing on these answers, this study, for the first time, provides new insights help to further advance this field of research. In a nutshell, the main contributions of this paper could be summarized as follows:

\begin{itemize}
	\item To the best of our knowledge, this work represents the first attempt to infer structure similarity between fitness landscapes of different COPs.
	\item We proposed a new fitness landscape visualization technique based on LON by leveraging node embedding and dimensionality reduction method.
    \item We developed a quantitative measure of structural similarity between different combinatorial landscapes using graph embedding technique and correlation metrics.
    \item We developed a \texttt{Python} package for performing graph-based landscape analysis. 
\end{itemize}

In the rest of this paper, \pref{sec:preliminaries} provides some preliminary knowledge related to this work. \pref{sec:method} delineates our empirical methodologies for problem instance generation and LON construction. Extensive empirical results are presented and analyzed in~\pref{sec:results}. In the end, \pref{sec:conclusions} concludes this paper and threads some light on future directions.

% The "No-Free-Lunch" Theorem
% Despite many successful BBOP solvers have been developed in different disciplines, the famous \enquote{No-Free-Lunch} theorem~\cite{DolpertM97} points out that there is no single algorithm that could always yield superior performance than others for all optimization problems. Therefore, in-depth understanding of the characteristics of the underlying BBOP is required to facilitate the design, selection as well as configuration of appropriate solvers for a given task.

% Under this paradigm, the task of finding an effective solver for a given problem instance could be transformed into the problem of finding a similar instance for which an effective solver is already known. At the core of this theory is a proper definition of the \textit{similarity} between problem instances, which is often based on representative features that are able to capture certain problem characteristics designed by domain experts.
% At the core of the analogical reasoning process is the judgement of \textit{similarity} between problems, which is often based on representative features that are able to capture certain problem characteristics designed by domain experts.

% While most of the existing works are dedicated to the study of a single type of BBOP, there has been evidence that the fitness landscapes of different BBOPs, although superficially different, may share certain patterns or sub-structures, rather than a full randomness~\cite{TayaraniP14}. 
% it is often the case that we are also interested in the relationship between different BBOP instances, i.e., is there any sharing of certain patterns or sub-structures among the fitness landscapes of different BBOPs?
% it is often the case that we are interested in the relationship between different problem instances. In fact, it has long been desired to answer the question of \enquote{what makes a BBOP hard?}. There have been attempts to classify BBOP instances into \enquote{hard} and \enquote{easy} ones~\cite{BrownNS09}. It has also been noted that although different at the surface, the fitness landscapes of different BBOPs may share certain patterns or structures, rather than a total disimilarity~\cite{TayaraniP14}. 

% Its fundamental premise is that if two problems share certain similarities with each other, then the problem-solving strategy effective for one problem would possibly also be useful for the other one. 
% In the context of BBOP, it is often the case in real world scenarios that we may encounter a problem instance which could be essentially similar to well-known problem. 

% \begin{figure}[t]
%     \centering
%     $\mathbf{S}=
%     \begin{blockarray}{*{4}{c} l}
%       \begin{block}{*{4}{>{$\footnotesize}c<{$}} l}
%         $P_0$ & $P_1$ & $P_2$ & $P_3$ & \\
%       \end{block}
%       \begin{block}{[*{4}{c}]>{$\footnotesize}l<{$}}
%         - & $\times$ & $\times$ & $\times$  \bigstrut[t]& $P_0$ \\
%         0.9 & - & $\times$ & $\times$  & $P_1$ \\
%         0.7 & 0.8 & - & $\times$  & $P_2$ \\
%         0.4 & 0.5 & 0.6 & -  & $P_3$ \\
%       \end{block}
%     \end{blockarray}$
%     \caption{An example of similarity matrix $\mathbf{S}$ for a set of four BBOP instances.}
%     \label{fig:similarity_matrix}
% \end{figure}

==> definitions.tex <==
%!TeX root=main.tex

\section{Preliminaries}
\label{sec:preliminaries}

In this section, we provide some important background knowledge and definitions pertinent to this paper. 

% Subsection 1: Problems 
% ----------------------


% Subsection 2: Fitness Landscape
% -------------------------------
\subsection{Fitness Landscapes}

\paragraph{Fitness landscapes} 
The original idea of \textit{fitness landscape} dates back to 1932 when Wright pioneered this concept in evolutionary biology~\cite{Wright1932}, and a formal expression was developed by Stadler as a triplet $(\mathcal{X},\mathcal{N},f)$~\cite{Landscape_Stadler}, where $\mathcal{X}$ is the space of potential solutions, $\mathcal{N}$ indicates a neighborhood structure that relates solutions in $\mathcal{X}$, and $f:\mathcal{X}\to{\mathbf{R}}$ is the fitness function of the underlying problem. For NPP, a solution in $\mathcal{X}$ can be represented as a vector binary string with a length $n$.

\paragraph{Local optimum} 
A solution is a \textit{local optimum} if its fitness value is superior to any other solution in its neighborhood. In other words, for a minimization problem like NPP, $\mathbf{x}^\ell$ is a local optimum if $\forall\mathbf{x}\in{\mathcal{N}(\mathbf{x}^\ell)}$, we have $f(\mathbf{x}^\ell)\leq{f(\mathbf{x})}$.

\paragraph{Basin of attraction} 
The \textit{basin of attraction} $\mathcal{B}$ of a local optimum $\mathbf{x}^\ell$ is the set of all solutions from which local search converges to $\mathbf{x}^\ell$, i.e., $\mathcal{B}=\{\mathbf{x}\in{\mathcal{X}}\mid\mathrm{LocalSearch}\rightarrow\mathbf{x}^\ell\}$.

\paragraph{Landscape Funnel}
Funnel of a fitness landscape is a global basin shape that includes some clustered local optima. Within these local optima, the optimal solution is located at the bottom of the funnel, surrounded by sub-optima solutions with gradually decreasing fitness. The paths leading from the surrounding local optima to the funnel bottom could be considered as a set down-hill trajectories that converge to the optima solution.

% Subsection 2: Fitness Landscape
% -------------------------------
\subsection{Local Optima Network}

A LON is considered as a subspace of fitness landscape constituted by local optima. It compresses the information of the whole search space into a graph $\mathcal{G}=(\mathcal{V},\mathcal{E})$, where the vertex set $\mathcal{V}$ consists of local optima and the edge set $\mathcal{E}$ indicates the transitions between them. As mentioned in~\pref{sec:previous_literature}, there exist various types of definitions of an edge in LONs. In this study, we consider escape edges, which do not require exhaustive enumeration of the search space. Instead, these edges account for the chances of escaping a local optimum after a controlled mutation (e.g. $2$-bit-flips in binary space) followed by hill-climbing. 



==> introduction_copy.tex <==

\section{Introduction}
\label{sec:introduction}


\IEEEPARstart{B}{lack-box} optimization problems (BBOPs), originated from black-box concepts in cybernetics, aims at finding a solution $\mathbf{x} \in \mathbb{R}^n$ that maximizes or minimizes an objective value $f(\mathbf{x})$ without any explicit knowledge of the objective function $f: \mathbb{R}^n \to \mathbb{R}$. Such problems are often encounterd in various scenarios in real-world engineering such as economics, machine learning and software engineering, etc. 
Despite many sucessful BBOP solvers have been developed in different disciplines, the famous \enquote{No-Free-Lunch} theorem~\cite{DolpertM97} points out that there is no single algorithm that could always yield superior perfromance than others for all optimization problems. Therefore, in-depth understanding of the characteristics of the underlying BBOP is essential to facilitate the design, selection and configuration of appropriate solvers for a given task. However, since there does not exist any analytical form or authentic solution for a BBOP, it is hard to interpret and investigate except for an observation of input-output response through experimentation.

In practice, analogy is one of the most common problem-solving approaches, and it is particularly helpful for the understanding of abtract, complex systems~\cite{RichlandS15}. In the context of BBOP, its basic assumption is that if a BBOP solver is effective for one problem, we could then expect its effectiveness for solving other problems which essentially share \textit{similarity} with each other. Thereby, when encountering a novel BBOP instance $P_0$, we could follow an analogical reasoning process to study it, which typically consists of three tasks~\cite{Gentner83, ThagardHNG90}:

\begin{itemize}
    \item \textit{Retrieval}: select a set of candidate analogous instances $\mathcal{P} = \{P_1, \dots, P_k\}$.
    \item \textit{Judgement}: determine the similarity $\mathrm{Sim}(P_i,P_j)$ between each distinct pair of instances  $(P_i, P_j)\in\mathcal{P}^2$ based on a similarity function $\mathrm{Sim}: \mathcal{P} \times \mathcal{P} \rightarrow [0, 1]$ (and thus obtain a similarity matrix $\mathbf{S}$ as shown in \pref{fig:matrix}).
    \item \textit{Inference}: apply knowledge from the most analogous instance $\hat{P_0}$ to handle $P_0$, where $\mathrm{Sim}(\hat{P},P) \geq \max_{P' \in \mathcal{P}} \mathrm{Sim}(P',P_0)$ for $\forall P' \in \mathcal{P}$. Here, the specific knowledge applied would depend on tasks at hand.
\end{itemize}

\begin{figure}[t!]
    \centering
    \includegraphics[width=.45\linewidth]{figs/matrix.pdf}
    \caption{An example of similarity matrix $\mathbf{S}$ for a set of BBOP instances $\mathcal{P} = \{P_0, \dots, P_3\}$. A \enquote{$-$} in the diagonal entry indicates that is is meaningless to measure the similarity of an instance with itself. The upper trangular part of the matrix is symmetric to the lower one and is thus omitted for brevity.}
    \label{fig:matrix}
\end{figure}

The inferrence of such similarity would not only enable us to transfer our knowledge on a well-studied problem to solve previously unseen instances, but also deepen our understanding of the relationships between different problem instances, and thus brings a fundamental new pespective for studying BBOPs. However, in practice it is far from trivial to directly infer such similarity when encountering BBOPs due to their black-box nature. 

In evolutionary and meta-heuristic optimization, the fitness landscape~\cite{Wright1932} metaphor and its analysis (known as fitness landscapes analysis, FLA) have been extensively used to understand the underlying properties of BBOPs. In particular, the \textit{structural characteristics} of BBOP landscapes are found to be able to reflect important properties of problem instances and indicative to the overall performance of heuristic solvers. This makes FLA a promising proxy for the inference of similarity between different BBOP instances. In other words, the strategic walk on the fitness landscapes of a solver might be extended to fitness landscapes 

In fact, there have been abundant evidence suggesting that certain patterns are associated with the landscape structure of a BBOP, and such patterns may share among different problem instances, or, even across different classess of problems~\cite{TayaraniP14}. However, despite many efforts, there has been no dedicated work to intuitively illustrate or quantitatively determine the \textit{structural similarity} between the fitness landscapes of different BBOP instances due to the lack of suitable analytical methods.

In the last three decades and beyond, considerable efforts have been devoted to developing statistical measures for characterizing fitness landscape, e.g., ruggendess, neutrality, epistasis variance and information content, etc. They have been successfully applied to guide the design and improvement of BBOP solvers, constitute feature vectors for automated algorithm selection and performance prediction, as well as gain insights into BBOPs themselves. However, in cogonitive science it is often the case that high-order relationships play a much more important role in determing the similarity between two instances. For example, whilst battery and reservoir are totally different things in many aspects (e.g., color, size shape and substance), at a higher level, their similary functions of storing and releasing energy makes it reasonble to consider them as analogous. It is thereby not sufficient to base our structural similarity inferrence only on hand-crafted features.

In the more recent decade, local optima networks (LONs) was proposed to model local optima in a fitness landscape and their transitions as a graph obejct. Specifically, the vertices of a LON are local optima and the edges indicate certain search dynamics of a meta-heuristic algorithm. Since LONs are able to capture various characteristics of the underlying landscape (e.g., the number of local optima, their distribution and connectivity pattern), they are powerful tools for fitness landscape analysis. In particular, the graph nature of LON makes it highly suitable for studying the structural characteristics of fitness landscapes. Notably, graph layout and node embedding techniques would enable us to obtain intuitive visualizations of the typological structures of fitness landscapes and make comparison between them~\cite{HuangL23}. In addition, Morever, graph representation learning techniques~\cite{ZhangYZZ20} are able to extract low-dimensional representations that could capture high-level structures of fitness landscapes, which have shown efficacy in the determination of structural similarity between different fitness landscapess~\cite{HuangL23}. 

% % point 1
% For example, metrics developed for complex networks~\cite{BoccalettiLMCH06} could be applied to analyze structural properties of the underlying landscapes. 
% % point 2
% In addition, graph layout and node embedding techniques would enable us to obtain intuitive visualizations of the typological structures of fitness landscapes~\cite{Graph_Visual_Survey1}.
% % point 3
% Morever, graph representation learning techniques~\cite{ZhangYZZ20} are able to extract low-dimensional representations that could capture high-level structures of fitness landscapes, which have shown efficacy in the determination of structural similarity between different fitness landscapes. 

Build on our recent work which conducted a case study on inferring the structural similarity of fitness landscapes across different dimensions of number partitioning problems (NPPs), in this study, we seek to gain further insights on a wider scope of landscapes with more comprehensive analysis. Specifically, we consider four types of classic BBOPs, inlcuding NPP, maximum satisfiability (Max-Sat), the traveling salesman problem (TSP), and the knapsack problem (KP). We seek to study the structural similarity of different problem instances at different levels, which lead us to our first three research questions (RQs). To start with, we also first consider problem instances of different dimensions. 

\begin{itemize}
    \item \textbf{\underline{RQ1}}: \textit{For each class of problems, can we investigate any potential structural similarity in fitness landscapes across instances of \underline{different dimensions?}}
    \item \textbf{\underline{RQ2}}: \textit{For each class of problems, can we investigate any potential structural similarity in fitness landscapes across instances of \underline{different sub-classes?}}
    \item \textbf{\underline{RQ3}}: \textit{Can we investigate any potential structural similarity in fitness landscapes across instances that belong to \underline{different classes} of problems?}
\end{itemize}

% \begin{tcolorbox}[sharpish corners, top=2pt, bottom=2pt, left=4pt, right=4pt, boxrule=0.0pt, colback=black!20!white, leftrule=0.75mm,]
%     \textbf{\underline{RQ1}:} \textit{For each class of problems, can we investigate any potential structural similarity in fitness landscapes across instances of different dimensions?}
% \end{tcolorbox}

% \begin{tcolorbox}[sharpish corners, top=2pt, bottom=2pt, left=4pt, right=4pt, boxrule=0.0pt, colback=black!20!white, leftrule=0.75mm,]
%     \textbf{\underline{RQ2}:} \textit{For each class of problems, can we investigate any potential structural similarity in fitness landscapes across instances of different sub-classes?}
% \end{tcolorbox}

% \begin{tcolorbox}[sharpish corners, top=2pt, bottom=2pt, left=4pt, right=4pt, boxrule=0.0pt, colback=black!20!white, leftrule=0.75mm,]
%     \textbf{\underline{RQ3}:} \textit{Can we investigate any potential structural similarity in fitness landscapes across instances of different classes of problems?}
% \end{tcolorbox}

The empirical results with regard to the first three RQs is highly inspiring, as we are able to disclose the similarities and differences between a wide range of instances by both qualitative and quantitative analysis. We then evalute the efficacy of our measured similarity by running heuristic algorithms on each problem instance. The rationale behind this particular analysis is based on the hypothesis that the level of similarity between two landscapes should be correlated with the performance difference of meta-heuristics on the corresponding problems, which leads to our final RQ: 

\begin{itemize}
    \item \textbf{\underline{RQ4}}: \textit{How effective is the measured similarity in explaining the performance difference of meta-heuristics between different problem instances?}
\end{itemize}

% \begin{tcolorbox}[sharpish corners, top=2pt, bottom=2pt, left=4pt, right=4pt, boxrule=0.0pt, colback=black!20!white, leftrule=0.75mm,]
%     \textbf{\underline{RQ4}:} \textit{How effective is the measured similarity in explaining the performance difference of meta-heuristics between different problem instances?}
% \end{tcolorbox}

The experimental results show that the $Sim$ value could has a good correlation with performance differences of testing algorithms.

Details of our empirical experiments and responses to these RQs will be elaborated in later sections step by step. Drawing on these answers, this study, for the first time, provides new insights help to further advance this field of research. In a nutshell, the main contributions of this paper could be summarized as follows:

\begin{itemize}
	\item To the best of our knowledge, this work represents the first attempt to infer structure similarity between fitness landscapes of different COPs.
	\item We proposed a new fitness landscape visualization technique based on LON by leveraging node embedding and dimensionality reduction method.
    \item We developed a quantitative measure of structural similarity between different combinatorial landscapes using graph embedding technique and correlation metrics.
    \item We developed a \texttt{Python} package for performing graph-based landscape analysis. 
\end{itemize}

In the rest of this paper, \pref{sec:preliminaries} provides some preliminary knowledge related to this work. \pref{sec:method} delineates our empirical methodologies for problem instance generation and LON construction. Extensive empirical results are presented and analyzed in~\pref{sec:results}. In the end, \pref{sec:conclusions} concludes this paper and threads some light on future directions.

% The "No-Free-Lunch" Theorem
% Despite many successful BBOP solvers have been developed in different disciplines, the famous \enquote{No-Free-Lunch} theorem~\cite{DolpertM97} points out that there is no single algorithm that could always yield superior performance than others for all optimization problems. Therefore, in-depth understanding of the characteristics of the underlying BBOP is required to facilitate the design, selection as well as configuration of appropriate solvers for a given task.

% Under this paradigm, the task of finding an effective solver for a given problem instance could be transformed into the problem of finding a similar instance for which an effective solver is already known. At the core of this theory is a proper definition of the \textit{similarity} between problem instances, which is often based on representative features that are able to capture certain problem characteristics designed by domain experts.
% At the core of the analogical reasoning process is the judgement of \textit{similarity} between problems, which is often based on representative features that are able to capture certain problem characteristics designed by domain experts.

% While most of the existing works are dedicated to the study of a single type of BBOP, there has been evidence that the fitness landscapes of different BBOPs, although superficially different, may share certain patterns or sub-structures, rather than a full randomness~\cite{TayaraniP14}. 
% it is often the case that we are also interested in the relationship between different BBOP instances, i.e., is there any sharing of certain patterns or sub-structures among the fitness landscapes of different BBOPs?
% it is often the case that we are interested in the relationship between different problem instances. In fact, it has long been desired to answer the question of \enquote{what makes a BBOP hard?}. There have been attempts to classify BBOP instances into \enquote{hard} and \enquote{easy} ones~\cite{BrownNS09}. It has also been noted that although different at the surface, the fitness landscapes of different BBOPs may share certain patterns or structures, rather than a total disimilarity~\cite{TayaraniP14}. 

% Its fundamental premise is that if two problems share certain similarities with each other, then the problem-solving strategy effective for one problem would possibly also be useful for the other one. 
% In the context of BBOP, it is often the case in real world scenarios that we may encounter a problem instance which could be essentially similar to well-known problem. 

% \begin{figure}[t]
%     \centering
%     $\mathbf{S}=
%     \begin{blockarray}{*{4}{c} l}
%       \begin{block}{*{4}{>{$\footnotesize}c<{$}} l}
%         $P_0$ & $P_1$ & $P_2$ & $P_3$ & \\
%       \end{block}
%       \begin{block}{[*{4}{c}]>{$\footnotesize}l<{$}}
%         - & $\times$ & $\times$ & $\times$  \bigstrut[t]& $P_0$ \\
%         0.9 & - & $\times$ & $\times$  & $P_1$ \\
%         0.7 & 0.8 & - & $\times$  & $P_2$ \\
%         0.4 & 0.5 & 0.6 & -  & $P_3$ \\
%       \end{block}
%     \end{blockarray}$
%     \caption{An example of similarity matrix $\mathbf{S}$ for a set of four BBOP instances.}
%     \label{fig:similarity_matrix}
% \end{figure}

==> makefile <==
FILE=main

all:	
	latex $(FILE)
	bibtex $(FILE)
	latex $(FILE)
	latex $(FILE)
	dvips -o $(FILE).ps $(FILE).dvi
	ps2pdf $(FILE).ps
	open $(FILE).pdf

clean:
	rm -f *.aux *.blg *.log *.bbl *.out *.bak *.synctex.gz *.synctex.gz\(busy\) *.tex~

cleanall: clean
	rm -f *.dvi $(FILE).ps $(FILE).pdf

